Learning Object Detection from Captions via Textual Scene Attributes

Object detection is a fundamental task in computer vision, requiring large annotated datasets that are difficult to collect, as annotators need to label objects and their bounding boxes. Thus, it is a significant challenge to use cheaper forms of supervision effectively. Recent work has begun to explore image captions as a source for weak supervision, but to date, in the context of object detection, captions have only been used to infer the categories of the objects in the image. In this work, we argue that captions contain much richer information about the image, including attributes of objects and their relations. Namely, the text represents a scene of the image, as described recently in the literature. We present a method that uses the attributes in this "textual scene graph" to train object detectors. We empirically demonstrate that the resulting model achieves state-of-the-art results on several challenging object detection datasets, outperforming recent approaches.

==> sections/setup.tex <==
\ignorebig{
\section{WSOD: The Learning Setup} 

In the WSOD task, we are given a bag of $n$ bounding boxes, $\mathcal{B}_1,...,\mathcal{B}_n$ and a bag of $m$ labels $\mathcal{L}_1,...,\mathcal{L}_m$, and the goal is to assign a bounding box $i$, $\mathcal{B}_i$ with a label $j$, $\mathcal{L}_j$. We followed the standard multiple instance (SMI) assumption~\cite{amores2013multiple}, every positive bag contains at lead one positive box instance, while in every negative bag all of the box instances are negative. We formulate is as follows: Given two sets $L$ and $B$ and a weight function $C: L \times B \to R$, find a bijection $f: B \to L$, such that the cost function is $\sum_{b \in B} C(b, f(b))$.	

A major concern is how to aggregate different predictions of the model for each of the bag instances. Most WSOD approaches utilize either mean or max pooling, the latter more frequently than the former~\cite{feng2017deep, pinheiro2015image, zhu2017deep}. The max pooling aggregation has attracted popularity due to its consistency with the SMI assumption: since a single instance is sufficient for classifying the entire bag, a high confidence value for either of the instances should derive a high confidence value for the entire bag. The downside of using these simple pooling functions is that they are not trainable, limiting their applicability. Other WSOD pooling operators contain global adaptive parameters, such as noisy-and~\cite{kraus2016classifying}. In this work, we use a variation of max pooling that is based both on the objects and attributes predictions.
}

==> sections/sg_loss.tex <==
\section{Scene Graph Entanglement Loss}
\label{chap:sg_loss}


% Image captions contain much richer data than object pseudo-labels. Namely, In addition to listing the objects that are present in the image, the captions can also tell us about the relations between the objects, their positions within the image and their visual attributes. A unified way to look at this additional information is well known in research as scene graphs, which are considered to be canonical representations that contain this data. In this work, we claim that by aligning the scene graph structure as extracted from the captions to the different image regions, we can provide the model with improved understanding of the visual scenes and get superior object detection results. 

Image captions can contain richer and more meaningful data than just object pseudo-labels. Namely, in addition to listing present objects in the image, the captions can suggest the relations between the objects, their positions within the image and even their visual attributes. A unified approach to look at this additional information is using scene graphs, which are considered canonical representations for containing this data. In this work, we claim that by aligning the scene graph structure as extracted from the captions to the different image regions, we can provide the model with an improved understanding of the visual scenes and get superior object detection results. 

Our proposed SG entanglement loss aims to predict the alignment between the textual scene graphs and the image regions. In this loss, in addition to the object classification layers, we also predict attribute scores for different attribute categories. Then, we use the attribute scores to aid the object detection learning process. For example, consider the image caption ``a red stop sign is glowing against the dark sky''. Instead of extracting only the ``stop sign'' object pseudo-label and discarding the rest of the caption information, we propose to use the ``red'' attribute label to enhance our supervision. Namely, instead of training the model to find the image region that is the most probable to be a ``stop sign'', our training objective is now to find the one that is the most probable to be both a ``stop sign'' and ``red''. An Illustration of the usage of the visual attributes in the object classification process is shown in Figure \ref{teaser}.

==> sections/wsod.tex <==
\section{Weakly Supervised Object Detection} 
\amirg{THis is a bit out of place. It's more like related work, so you can expand a bit in the related work section, but I think we can skip this section and just integrate whatever we need from it when we describe our approach.}
\label{chap:wsod}

Object detection has many real-life applications, both by itself and as a basis for other computer vision capabilities. The problem of \textit{weakly supervised object detection}\roei{Add cite.} has emerged from the natural need to alleviate the expensive requirement for a manually large-scale labeled dataset. Therefore, the WSOD task is even more challenging than regular object detection, as the trained model does not use bounding boxes annotations to learn from. Despite extensive research over the past years, WSOD remains an open problem, as indicated by the large performance gap of $\sim$20\% between WSOD~\cite{tang2017multiple,wan2018min,wei2018ts2c} and fully supervised detection approaches~\cite{ren2015faster} on the PASCAL VOC detection benchmark~\cite{everingham2010pascal}.

% In this work, we tackle the problem of training an object detector from image captions from a WSOD point of view, i.e., the object labels are extracted from the captions in an "offline" manner. We show that this simplistic approach does not efficiently utilize the image captions, and a smarter SG data extraction could improve the performance of the model.

\textbf{Multiple Instance Learning.} WSOD is a specific task out of a broader class of problems, named \textit{Multiple Instance Learning} (MIL). In MIL problems, instead of receiving a set of individually labeled instances, the learner receives a set of labeled bags, each containing many instances \cite{dietterich1997solving}. In particular, MIL is a valuable formalization for problems with a high input complexity and weak forms of supervision, such as medical images processing~\cite{quellec2017multiple}, action recognition in videos~\cite{ali2008human} and sound event detection~\cite{kumar2016audio}. The motivation of the MIL formalization stems from the fact that the correct label for the input bag can be predicted from a single instance. For example, in the WSOD task, an object can be inferred from the specific image patch in which the object appears. This is referred to as the standard multiple instance (SMI) assumption~\cite{amores2013multiple}, i.e., every positive bag contains at least one positive instance, while in every negative bag all of the instances are negative.

% For example, in WSOD the presence of an object in a image can be inferred from the specific image patch in which the object appears. This is referred to as the standard multiple instance (SMI) assumption: every positive bag contains at least one positive instance, while in every negative bag all of the instances are negative \cite{amores2013multiple}. The MIL problem has, therefore, attracted a considerable amount of research efforts.

A major concern is how to aggregate different predictions of the model for each of the bag instances. Most MIL approaches utilize either mean or max pooling, the latter more frequently than the former ~\cite{feng2017deep, pinheiro2015image, zhu2017deep}. The max pooling aggregation has attracted popularity due to its consistentcy with the SMI assumption: since a single instance is sufficient for classifying the entire bag, a high confidence value for either of the instances should derive a high confidence value for the entire bag. The downside of using these simple pooling functions is that they are not trainable, limiting their applicability. Other MIL pooling operators contain global adaptive parameters, such as noisy-and \cite{kraus2016classifying}. In this work, we use a variation of max pooling that is based both on the objects and attributes predictions.



% A major question in MIL is how to aggregate the different predictions of the model for each of the instances in the bag. Most MIL approaches utilize either mean or max pooling, the latter more frequently than the former \cite{feng2017deep} \cite{pinheiro2015image} \cite{zhu2017deep}. Usage of max pooling is in fact consistent with the SMI assumption - since a single instance is sufficient for classifying the entire bag, a high confidence value for either of the instances should derive a high confidence value for the entire bag. The downside in using these simple pooling functions is that they are not trainable, which potentially limits their applicability. There are MIL pooling operators that contain global adaptive parameters, such as noisy-and \cite{kraus2016classifying}. In this work, we use a combination of regular max pooling and a SG-based max pooling.




